The Explosion in Orion-KL as Seen by Mosaicking the Magnetic Field with ALMA

We present the first linear-polarization mosaicked observations performed by the Atacama Large Millimeter/submillimeter Array (ALMA). We mapped the Orion-KLeinmann-Low (Orion-KL) nebula using super-sampled mosaics at 3.1 and 1.3 mm as part of the ALMA Extension and Optimization of Capabilities (EOC) program. We derive the magnetic field morphology in the plane of the sky by assuming that dust grains are aligned with respect to the ambient magnetic field. At the center of the nebula, we find a quasi-radial magnetic field pattern that is aligned with the explosive CO outflow up to a radius of approximately 12 arc-seconds (~ 5000 au), beyond which the pattern smoothly transitions into a quasi-hourglass shape resembling the morphology seen in larger-scale observations by the James-Clerk-Maxwell Telescope (JCMT). We estimate an average magnetic field strength $\langle B\rangle = 9.4$ mG and a total magnetic energy of 2 x 10^45 ergs, which is three orders of magnitude less than the energy in the explosive CO outflow. We conclude that the field has been overwhelmed by the outflow and that a shock is propagating from the center of the nebula, where the shock front is seen in the magnetic field lines at a distance of ~ 5000 au from the explosion center.

==> ms_header.tex <==

%%%%%%%%%%%%%%
% Short cuts %
%%%%%%%%%%%%%%

% Astrometry Units

\newcommand{\hr}{\mbox{$^h$}}
\renewcommand{\min}{\mbox{$^m$}}
\renewcommand{\sec}{\mbox{$^s$}}
\renewcommand{\deg}{\mbox{$^{\circ}$}}
%\newcommand{\arcmin}{\mbox{$^'$}}
%\newcommand{\arcsec}{\mbox{$^{''}$}}
\newcommand{\kms}{\mbox{km\,s$^{-1}$}}
\newcommand{\fluxunits}{\mbox{erg\,cm$^{-2}$ s$^{-1}$}}
\newcommand{\uJy}{\mbox{$\mu$Jy}}
\newcommand{\um}{\mbox{$\mu$m}}
\newcommand{\ULL}{\mbox{$<27.0$}}
% Miscellaneous
\newcommand{\dbrk}{\mbox{$D(4000)$}}
\newcommand{\wrst}{\mbox{$W_{\lambda}^{\mbox{\tiny rest}}$}}
\newcommand{\wrsti}{\mbox{$W_{\lambda,i}^{\mbox{\tiny rest}}$}}
\newcommand{\wobs}{\mbox{$W_{\lambda}^{\mbox{\tiny obs}}$}}
\newcommand{\haln}{\mbox{H$\alpha$(n)}}
\newcommand{\halb}{\mbox{H$\alpha$(b)}}
\newcommand{\simgtr}{\, \raisebox{-.2ex}{$\stackrel{>}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\simlt}{\, \raisebox{-.2ex}{$\stackrel{<}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\sigsky}{\mbox{$\sigma_{\mbox{\tiny sky}}$}}
\newcommand{\bootes}{Bo\"{o}tes}
\newcommand{\lamfwhm}{\mbox{$\Delta \lambda_{\mbox{\tiny FWHM}}$}}
\newcommand{\lamblaze}{\mbox{$\lambda_{\mbox{\tiny blaze}}$}}
\newcommand{\rarrow}{\mbox{$\Rightarrow$}}
\newcommand{\fshrt}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny short}}$}}
\newcommand{\flng}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny long}}$}}
\newcommand{\ztit}{\mbox{$z \approx 4.5$}}
\newcommand{\x}{\mbox{$\times$}}
\newcommand{\Msun}{\mbox{M$_{\odot}$}}
\newcommand{\Mdot}{\mbox{$\dot{m}_{-4}$}}
\newcommand{\Lsun}{\mbox{L$_{\odot}$}}
\newcommand{\E}[1]{\hbox{$10^{ #1 }$}}
\newcommand{\per}[1]{\hbox{#1$^{-1}$}}
\newcommand{\tothe}[1]{\hbox{$^{#1}$}}
\newcommand{\about}{\mbox{$\sim$}}
\newcommand{\SIG}{\mbox{W~m$^{-2}$~Hz$^{-1}$~sr$^{-1}$}}
\newcommand{\nISM}{\mbox{$n_{\rm ISM}$}}
%\newcommand{\uJy}{\mbox{$\mu$Jy}}
%\newcommand{\about}{\mbox{$\sim$}}
\def\IRAS       {\hbox{\it IRAS}}
\def\NVSS       {\hbox{\it NVSS}}

\def\OIII       {\hbox{O\tiny{III}}}
\def\NII        {\hbox{N\tiny{II}}}
\def\NO         {\hbox{---}}
\def\HII        {\hbox{H \small{II}}}
\def\Htwo       {\hbox{H_{2}}}
\def\HI         {\hbox{H \small{I}}}
\def\Ha         {\hbox{H \small{$\alpha$}}}
\def\Hb         {\hbox{H \small{$\beta$}}}
\def\SFIR       {\hbox{$S_{\rm FIR}$}}
\def\HCOP       {\hbox{HCO$^{+}$}}
\def\thirCO     {\hbox{$^{13}$CO}}
\def\water      {\hbox{H$_{2}$O}}
\def\source     {\hbox{G30.79\,FIR\,10}}

